Towards a Holistic and Automated Evaluation Framework for Multi-Level Comprehension of LLMs in Book-Length Contexts

We introduce HAMLET, a holistic and automated framework for evaluating the long-context comprehension of large language models (LLMs). HAMLET structures source texts into a three-level key-fact hierarchy at root-, branch-, and leaf-levels, and employs query-focused summarization to evaluate how well models recall and faithfully represent information at each level. To validate the reliability of our fully automated pipeline, we conduct a systematic human study, showing that our automatic evaluation achieves over 90% agreement with expert human judgments, while reducing the cost by up to 25 times. HAMLET reveals that LLMs struggle with fine-grained comprehension, especially at the leaf level, and are sensitive to positional effects like the lost-in-the-middle. Analytical queries pose greater challenges than narrative ones, and consistent performance gaps emerge between open-source and proprietary models, as well as across model scales. Our code and dataset are publicly available at https://github.com/DISL-Lab/HAMLET.

==> 2-introduction_original.tex <==
\section{Introduction}\label{sec:introduction}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/1-longdoc_overview_v3.pdf}
    \vspace{-0.7cm}
    \caption{The overview of \algname{} pipeline.}
    % \caption{The overview of \algname{} pipeline. The process flows left to right: (1) Source Data Preparation: novels exceeding 100K tokens are chunked into 4K-token segments for processing; (2) Perspective-specific Key-fact Tree Generation: LLMs construct hierarchical knowledge representations from analytical (logical reasoning) and narrative (storytelling) perspectives, with validator LLMs ensuring quality; (3) Query Generation: LLMs create perspective-aligned queries based on book chunks and their key-fact trees; (4) Summary Generation: LLMs produce summaries responding to both analytical and narrative queries; (5) Fine-grained Evaluation: summaries are assessed against key-fact trees and their corresponding chunks using multi-dimensional metrics (faithfulness, conciseness, completeness) at both sentence and key-fact levels, enabling detailed analysis of summary quality.}
    \label{fig:overview}
\vspace{-0.05cm}
\end{figure*}


% First, \textit{limited evaluation scope}: existing frameworks for evaluating LLMs' understanding of book-length contexts primarily rely on short-form generation tasks such as question-answering (QA) and multiple-choice evaluations, exemplified by benchmarks like LEval \cite{an-etal-2024-leval}, NovelQA \cite{wang2024novelqa}, and Nocha \cite{karpinska-etal-2024-onethousand_nocha}. These assessments depend on concise responses and discrete correctness metrics, insufficient for capturing the nuanced quality spectrum inherent in long-form outputs. Thus, there is a critical need for evaluation frameworks explicitly designed for open-ended, long-form generation tasks that extend assessment criteria beyond factual accuracy to include multiple dimensions.

% Second, \textit{reference-dependent assessment}: Although benchmarks such as BookSum \cite{kryscinski-etal-2022-booksum}, LooGLE \cite{li-etal-2024-loogle}, and {$\infty$Bench} \cite{zhang-etal-2024-infinitebench} address long-form generation and particularly summarization, they commonly evaluate quality by comparing outputs to fixed, single reference summaries presumed definitive. This overlooks summarization's multifaceted nature, where different summary purposes significantly impact what content is deemed salient—an issue magnified in long, complex book-length contexts. While a recent benchmark BoookScore \cite{chang2024booookscore} does not use a reference summary for evaluation, it focuses solely on logical structure and readability of generated summaries, neglecting crucial dimensions such as factual faithfulness. Moreover, although reference-free, multi-dimensional summarization evaluation frameworks such as G-Eval~\cite{liu2023geval} and FineSure~\cite{song2024finesure} exist, their applicability to book-length texts remains unexplored as the substantial volume and complexity of these texts present new challenges that extend beyond their original evaluation scope.


Recent advancements in large language models (LLMs) have expanded input capacities beyond 100K tokens—comparable to short novels. While facilitating novel applications, this expansion introduces challenges for evaluating LLM outputs from extensive inputs. Specifically, we identify three critical evaluation challenges: (1) \textit{limited evaluation scope}, (2) \textit{reference-dependent assessment}, and (3) \textit{scalability constraints}.

First, \textit{limited evaluation scope}: existing frameworks for evaluating LLMs' understanding of book-length contexts primarily rely on short-form generation tasks (\emph{e.g.}, question-answering (QA) and multiple-choice evaluations), exemplified by benchmarks such as NovelQA \cite{wang2024novelqa}, Nocha \cite{karpinska-etal-2024-onethousand_nocha}, and RULER~\cite{cheng-ping-etal-2024-ruler}. They rely on concise answers and discrete correctness metrics, which is insufficient for capturing the nuanced quality spectrum inherent in long-form outputs. Thus, there is a need for evaluation frameworks explicitly designed for open-ended, multidimensional long-form evaluation.

Second, \textit{reference-dependent assessment}: although benchmarks such as BookSum \cite{kryscinski-etal-2022-booksum}, LooGLE \cite{li-etal-2024-loogle}, and {$\infty$Bench} \cite{zhang-etal-2024-infinitebench} address long-form generation and particularly summarization, they typically compare outputs against fixed reference summaries. This approach overlooks the inherent complexity of summarization, where different purposes dictate varying content priorities—particularly critical in lengthy, complex contexts. Furthermore, multi-dimensional evaluation frameworks such as G-Eval~\cite{liu2023geval} and FineSure~\cite{song2024finesure} have yet to explore their applicability for book-length contexts.

Third, \textit{scalability constraints}: current benchmark pipelines for book-length contexts struggle to operate efficiently at scale. Creating evaluation datasets depends heavily on labor-intensive human annotation \cite{an-etal-2024-leval, li-etal-2024-loogle, wang2024novelqa,  karpinska-etal-2024-onethousand_nocha}, making benchmark creation costly and time-consuming, especially for book-length texts.  This exacerbates the risk stemming  from data leakage, where newer models trained on benchmark data quickly render static benchmarks obsolete. 
Consequently, there is a pressing need for adaptable and scalable evaluation \textit{pipeline} that can generate benchmark instances with minimal or no human intervention.

To address these challenges, we propose \algname{} (Figure~\ref{fig:overview}), a scalable benchmark pipeline designed explicitly for evaluating the open-ended, long-form generation capability of LLMs on book-length contexts. \algname{} builds upon the task of Query-focused Summarization (QFS), which is defined as a task of generating summaries tailored to specific queries. The key advantage of the QFS framework in addressing the identified challenges is that it allows LLMs to emphasize dynamically diverse aspects of the input document based on the query posed, which is crucial for addressing book-length contexts where the thematic transition is frequent. To adapt this QFS framework more aptly with the evaluation of the long-form, open-ended generation abilities of LLMs on book-length contexts, \algname{} introduces two novel components enhancing QFS' effectiveness.

First, we incorporate dual summarization perspectives—\textit{analytical} and \textit{narrative}—into query generation of QFS framework in the novel domain (Table~\ref{tab:perspective-comparison}), explicitly evaluating summaries under contrasting summary requirements. While other summarization perspectives could exist, we specifically limit our scope to these two, defined respectively as focusing on logical reasoning (analytical), and storytelling (narrative). This representative yet comprehensive choice provides deeper insights into how LLMs adapt summaries according to diverse query intents.

% First, we introduce a detailed strategy for systematically integrating various \textit{summarization perspectives} into the QFS framework. Our research specifically focuses on the novel domain, implementing dual summarization perspectives—analytical and narrative—in our query generation process (Table~\ref{tab}). These two perspectives are deliberately selected to construct the foundation of our pipeline, enabling us to evaluate summaries under contrasting requirements: analytical perspectives emphasize logical reasoning, while narrative perspectives prioritize storytelling elements. Although additional summarization perspectives exist, we deliberately limit our scope to these two complementary dimensions in this study. This targeted yet comprehensive approach provides valuable insights into how LLMs adapt their summaries to accommodate diverse query intents when processing book-length texts.

Second, to enable a more structured evaluation of the generated summaries, we propose a novel hierarchical representation of information in the input context termed the \textit{key-fact\footnote{A key-fact is defined as a concise statement capturing critical information with at most 2–3 entities \cite{song2024finesure},} tree} (Table~\ref{tab:hierarchy-comparison}). Each key-fact is organized into hierarchical levels (root, branch, and leaf). The root represents the core informational theme pertinent to the query, branches specify major supporting elements, and leaves detail finer-grained information. These key-fact trees are specifically constructed to align with our dual summarization perspectives, with analytical queries generating fact trees focused on logical structures and implications, while narrative queries produce trees that emphasize chronological or sequential storyline. Each key-fact tree uniquely aligns with a specific query, serving as a structured answer sheet delineating essential content that must be reflected in the generated summaries, thus enabling detailed evaluation.

To eliminate dependency on reference summaries and human evaluation, \algname{} integrates the well-established multi-dimensional summary evaluation framework of \citet{song2024finesure}, which assesses faithfulness, completeness, and conciseness of generated summaries. This integration with our dual summarization perspectives and hierarchical key-fact trees extends current benchmarking capabilities in vital ways—enabling precise evaluation of model adaptability to different query intents while providing fine-grained analysis of information retention across hierarchical levels. Together, these advances in benchmarking paradigm directly address the identified challenges in existing benchmarks, creating an effective and scalable framework for evaluating long-form generation on book-length contexts~\ref{sec:humanval}. 

Crucially, our pipeline—covering query generation, key-fact tree construction, and summary evaluation—is \textit{fully automated} via LLMs, directly addressing scalability issues by removing human intervention. We rigorously assess the validity of the automated components through expert examination, ensuring the robustness of our pipeline robustness.

Our main contributions can be summarized as follows: (1) We introduce \textbf{a novel hierarchical summarization evaluation framework} that integrates QFS with varying summarization perspectives. It enables multi-dimensional assessment of long-form generation quality; (2) we develop \textbf{a fully automated, scalable benchmark pipeline} that eliminates the need for human annotation, making it adaptable to evolving models while maintaining robustness through expert validation; (3) we conduct \textbf{an in-depth analysis of open-ended, long-form generation abilities of LLMs within book-length contexts}, exploring how they adapt to varying query intents, maintain fidelity across different informational granularities, and handle the complexities inherent in book-length texts. 





==> 4-method_original.tex <==
\section{\algname{} Construction Pipeline}\label{sec:pipeline}

\begin{table*}[ht!]
  \centering
  \scriptsize{}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}
     >{\centering\arraybackslash}m{0.12\textwidth}  % first column, vertically centered
     M{0.4\textwidth}                               % Analytical
     M{0.4\textwidth}                               % Narrative
  }
  \toprule
  & \multicolumn{1}{c}{Analytical}
    & \multicolumn{1}{c}{Narrative} \\
  \midrule
  Definition
    & Analytical perspective focuses on thematic elements, implications, character development, and symbolic patterns, examining how these literary components build toward deeper meaning and authorial intent.
    & Narrative perspective emphasizes chronological storytelling, key events, and plot developments, concentrating on how the storyline unfolds and progresses through the text. \\
  \midrule
  Query Example
    & How do the social rejection and personal challenges Holmes faces at the bar, his subsequent return home with Callie Brett's assistance, and the professional and personal challenges faced by Poe and Holmes, including the discovery of twins, collectively illustrate the overarching themes of vulnerability, trust, and commitment in the narrative?
    & Provide a detailed summary of the events involving Holmes at the bar, his interaction with Callie Brett, the subsequent health incident, and the developments with Poe and Grey, including their medical appointment and the team's commitment to a crime-writers' convention? \\
  \bottomrule
  \end{tabular*}
  \caption{Definitions of two summarization perspectives and their example queries.}
  \label{tab:perspective-comparison}
\end{table*}

%%% main body %%%
We construct \algname{} following the systematic pipeline of five steps, as described in Figure~\ref{fig:overview}: (1) Source Data and Chunking; (2) Hierarchical and Multi-Perspective QFS Construction; (3) Summary Generation, and; (4) Fine-grained Summary Evaluation. In what follows, each step is described in detail.

\subsection{Step 1: Source Data and Chunking}\label{sec:source_data_prep}

% To construct \algname{}, we first collect 16 novels, called seed novels, with the average length of 101K tokens.
% All seed novels are published after June 2024, which is after the most recent training knowledge of the LLMs evaluated in \algname{} (see Appendix~\ref{tab:model_overview}. This ensures that our evaluation is not affected by data leakage.

To construct \algname{}, we first collect 16 novels, called seed novels, which are the recently published books  with the average length of 101K tokens.

% Note that the choice of the novel domain is not essential as \algname{} can be easily adapted and scaled to new data. However, it is effective for evaluation because it provides naturally occurring narrative structures with complex character relationships, themes, and plot developments---making it an ideal test for an LLM's ability to process and synthesize coherent pieces of long-form writing.

% To make the evaluation on book-length contexts controllable, we segment each novel into sequential 4K-token chunks. Each chunk serves as an evaluation unit for generating distinct query-summary pairs. This chunking strategy offers important evaluation advantages by enabling a manageable and interpretable analysis of query-specific understanding at different locations within a book-length context. Furthermore, since we maintain the sequential ordering of chunks, our chunking approach enables systematic positional analysis of how LLMs' comprehension abilities vary across different sections of book-length contexts.

In \algname{}, we adopt a chunking strategy that segments each book-length document into sequential 4K-token units, which serve as the foundation for both evaluation and supervision. This design is motivated by the inherent difficulty of constructing reliable and targeted evaluation signals over extremely long contexts.

Specifically, generating meaningful, comprehension-oriented queries and their corresponding key-fact trees directly from a 100K-token document is impractical—both for automated systems and human annotators. By restricting the supervision scope to a single chunk, we enable focused query generation and structured key-fact extraction that are grounded in a manageable, semantically coherent unit of text. Importantly, each chunk also serves as the exclusive evidence source during evaluation. This ensures that generated summaries are assessed only against the information that would have been accessible during supervision, avoiding the impact of the extreme long document. Furthermore, since we maintain the sequential ordering of chunks, our chunking approach enables systematic positional analysis of how LLMs' comprehension abilities vary across different sections of book-length contexts.
The detailed information on the seed novels and the generated chunks can be found in Appendix~\ref{appendix: dataset_statistics}.


\subsection{Step 2: Key-fact Tree and Multi-perspective Query construction}
\label{sec:key_fact_tree}
\paragraph{Overview.}

This step generates hierarchical key-fact trees tailored to different summary perspectives, forming the backbone of our evaluation framework. It consists of three components: (1) key-fact tree generation (Section~\ref{sec:tree_generation}); (2) query generation (Section~\ref{sec:query_generation}). 
% (1) summary perspectives (Section~\ref{sec:sum_perspective}); (2) key-fact tree generation (Section~\ref{sec:tree_generation}), and; (3) key-fact tree validation (Section~\ref{sec:tree_validation}).

% \subsubsection{Summary Perspectives}\label{sec:sum_perspective}
\paragraph{Summary Perspectives}\label{sec:sum_perspective} 
LLMs often exhibit varying comprehension ability depending on the perspective and granularity of the summary, even applied to the same document \cite{fonseca-cohen-2024-large-language}. This variability becomes more prominent in book-length contexts where the content is more dynamic and complex. These conditions underscore the importance of evaluating summarization performance under distinct interpretive objectives, rather than relying on a single summary formulation.
% This underscores the need to conduct separate analyses of summary from various perspectives.

In this paper, we identify two summary perspectives—\textit{analytical} and \textit{narrative} (see Table~\ref{tab:perspective-comparison}). These perspectives capture fundamentally different modes of novel comprehension. The analytical perspective focuses on themes, implications, and logical relationships between events, while narrative perspective emphasizes plot progression, character development, and sequential storytelling. By evaluating model performance under both perspectives, we aim to systematically assess the ability of LLMs to adapt their summarization strategies to varying semantic goals—a critical capability for navigating the rich structural and discourse complexity of book-length inputs.
% By evaluating LLMs performance under both perspectives, we can systematically assess their ability to adapt summarization strategies based on interpretive requirements—a critical capability when processing complex book-length texts with multiple interconnected themes and storylines.

While this study focuses on analytical and narrative perspectives tailored to the novel domain, the framework is extensible to other settings. For example, argumentative or decision-focused perspectives may be more appropriate in dialogue or instructional domains, allowing the framework to generalize across diverse document types.
% Note that, in this study we limit the summary perspectives to analytical and narrative which are tailored with the novel domain, but they can be adjusted for other domains (e.g, an argument-focused perspective for dialogues).

\subsubsection{Key-fact Tree Generation}\label{sec:tree_generation}

% The key‐fact tree translates a 4K‑token chunk of source text into a concise, hierarchical map of “what matters” for a given perspective. A tree may have multiple roots (independent high‑level ideas).  Every non‑leaf node typically expands into 1–4 children. Below we detail the design choices and the automatic procedure used to produce the trees.
To structure the evaluation of long-context summarization, we introduce a three-tier key-fact tree that distills each 4K-token chunk into a compact, interpretable representation of salient content. Tailored to the summarization perspective (analytical or narrative), this tree reflects both the semantic importance and granularity of information that a summary should convey.

\paragraph{Why a hierarchy?} A relation‑agnostic (flat) list of key-facts forces evaluators to weight all details equally, blurring the distinction between high‑level insight and granular evidence. 

By contrast, our three‑tier hierarchy mirrors the way expert readers organize information—first extracting an overarching idea, then assembling  mid‑level supports, and finally citing concrete textual proof.
This structure (i) exposes the logical backbone that links summary sentences to source evidence, (ii) supports fine‑grained error localization during evaluation, and (iii) enables the evaluation of an LLM’s ability to reason across multiple abstraction levels instead of merely transcribing every salient sentence.

By grounding every evaluation object in this compact, interpretable hierarchy, \algname{} moves beyond surface‑level overlap metrics and toward a principled assessment of long‑context reasoning.


% \paragraph{Schema.} Each key-fact tree comprises:


% \begin{itemize}
%   \item \textbf{Roots.} One or more nodes capturing the central analytical themes or pivotal narrative events of the chunk.
%   \item \textbf{Branches.} For each root, typically 1–3 nodes that refine it—major supporting elements in the analytical view, or primary plot elements in the narrative view.
%   \item \textbf{Leaves.} For each branch, typically 1–3 concrete, non‑redundant snippets (scenes, quotations, literary devices) that substantiate that branch.
% \end{itemize}

Traversing any root–branch–leaf path therefore yields a coherent  “claim $\rightarrow$ support $\rightarrow$ evidence” chain, which can later be aligned to generated summaries. See Table~\ref{tab:hierarchy-comparison} for detailed definitions and examples for each summarization perspective.

\paragraph{Automatic generation with GPT‑4o.} Given a chunk of a novel and a target perspective (analytical or narrative), we prompt GPT-4o (see Tables~\ref{tab:narrative_tree_generation} and \ref{tab:analytical_tree_generation}) to output a JSON‑like structure that is convertible into a directed tree. The prompt supplies: (1) a role description explaining the three‑level schema; (2) an exemplar (one per perspective) of well‑formed trees; (3) a chunk of a novel with 4,000 tokens, and; (4) perspective‑specific instructions. We set \texttt{temperature}$\approx$0 for determinism and reject outputs that violate the schema and re‑prompt them. All resulting key-fact trees are called \textit{raw key-fact trees}, which are then passed to the validation stage~\ref{sec:tree_validation}.


% \subsubsection{Validation of the Key‑fact Trees.}\label{sec:tree_validation}
\paragraph{Validation of the Key‑fact Trees.}\label{sec:tree_validation}
The \textit{raw key-fact trees} produced solely by a single prompting may contain hallucinations, subjective guesses, or trivial details. Therefore, to guarantee that only reliable information is retained, we run every key‑fact through a three‑dimension filter: (1) \textit{Faithfulness}:  the fact must be fully supported by the source chunk; (2) \textit{Objectivity}:  the wording must be objective without speculative language or value judgments; (3) \textit{Significance}:  the fact must add essential insight for the chosen perspective rather than restating minor information.

We configure GPT‑4o as a specialized validator for each dimension, prompting it separately for faithfulness, objectivity, and significance. Thus, every key‑fact tree undergoes three distinct validation passes—one per dimension—each supplied with the chunk text, the raw tree, and the corresponding instruction set shown in Tables~\ref{tab:keyfact_tree_validation_faith}–\ref{tab:keyfact_tree_validation_subj}.

After the three passes, the model’s \texttt{PASS}/\texttt{FAIL} judgments are merged: any key‑fact that fails even one dimension is deleted, and any descendant left without a valid parent is recursively pruned. This multi‑pass procedure keeps our trees faithful, objective, and significant, providing a solid foundation for the downstream query generation and summary evaluation stages. As a result, we obtain a total of 22,333 key-facts (including all roots, branches, leaves; see Appendix~\ref{appendix: dataset_statistics} for detailed statistics) across 16 novels.

% \subsubsection{Formal expression.}-> skip for now


\subsubsection{Query Generation}\label{sec:query_generation}

In this step, for each 4K‑token chunk, we generate \emph{two} perspective‑aligned queries—one analytical, one narrative—using its validated key‑fact tree. GPT‑4o is given the chunk and tree, and instructed to: (1) generate a single, self‑contained question whose answer necessarily weaves together the root, branch, and leaf key-facts; (2) keep the wording natural and specific to the chunk, and; (3) target the requested perspective— thematic chains for analytical queries and chronological explanation for narrative queries.

This procedure yields queries that precisely pinpoint specific information relevant to each chunk, effectively guiding summarization systems to locate and synthesize corresponding content within extensive book-length contexts. In total, we generate 814 queries across 16 novels (a total of 407 chunks × two summarization perspectives). Table~\ref{tab:perspective-comparison} provides examples of the generated queries for each summarization perspective. 


\subsection{Step 3: Summary Generation}\label{sec:summary_generation}

To investigate how long-form generation capabilities vary across different model scales and architectures, we evaluate six representative LLMs. These range from commercial models (GPT-4o, GPT-4o-Mini, Claude-3.5-Sonnet, and Claude-3.5-Haiku) to open-source models (Llama-3.1-405B-Instruct and Llama-3.1-8B-Instruct), which also allows for a direct comparison of parameter scales. Further model details are provided in Appendix~\ref{appendix:model_details}.

Each model receives the query together with the full novel, and the summary is generated by directly answering the queries. While the entire novel is visible, the generated summaries are expected to focus on the chunks from which the queries are derived. In total, we generate 4,800 summaries (16 novels × 25 chunks × 2 perspectives × 6 summarizers).


\subsection{Step 4: Fine-grained Summary Evaluation}\label{sec:summary_evaluation}

Since our goal is an automated benchmark pipeline, we leverage LLM‑based evaluators. Previous studies have shown that LLM evaluators exhibit comparable performance with human judgments~\cite{liu2023geval, wang2023chatgpt, tang2024minicheck, van2024field, fu2024gptscore, song2024finesure}. However, popular criteria such as "coherence" or "relevance" are too coarse for long‑context summarization—they cannot be turned into consistent quantifiable scores. We therefore follow the FineSurE protocol~\cite{song2024finesure} and rate each summary along three concrete axes: \textit{faithfulness}, and \textit{completeness}.

Specifically, there are two evaluation tasks: \textit{fact verification}, where each sentence is compared with the chunk and marked correct or incorrect using the error types of~\citet{lee2024unisumeval} (see Table~\ref{tab:error-categories} for the details); and \textit{key‑fact alignment}, where every root, branch, and leaf key-fact is checked for entailment in the summary, mirroring a standard NLI judgment. Final scores are computed as follows: (1) \textit{Faithfulness} measures the percentage of summary sentences without factual errors; (2) \textit{Completeness} is the percentage of key-facts contained in summary sentences of key‑facts fully covered (see Appendix~\ref{appendix:eval_details} for the formal expressions).

Crucially, since the evaluation is based on key-fact trees that contain the information of varying detail, the completeness dimension can be assessed in even more fine-grained manner. Furthermore, 
all evaluation occurs at the chunk level. This eliminates the need to prompt the auto-evaluator with the entire novel, which can increase the risk of evaluation error and computation. This fosters effective and scalable summarization evaluation for book-length contexts. As a result, we generate a total of 83,693 automated labels from fact verification task, and 134,046 labels from key-fact alignment task.














% %%%%%%% old %%%%%%%%%%
% \paragraph{Summary Perspectives}
% % In this work, we address the challenges posed by lengthy source texts by introducing a chunking strategy with two main steps. First, we clean each novel by removing sections unrelated to the main text—such as the table of contents, author introductions, and publisher information. Second, we segment each novel from the beginning into consecutive 4K-token chunks, ensuring that no sentence is split across chunk boundaries. These shorter chunks enable large language models to effectively handle extensive content while preserving crucial context. Each chunk is then used to automatically generate content-relevant queries and to serve as evidence when evaluating the corresponding summaries. By applying this method to 16 novels, we produced a total of 407 chunks for subsequent experimentation and analysis.

% LLMs often exhibit varying comprehension ability depending on the perspective and granularity of the summary, even for the same document.\cite{fonseca-cohen-2024-large-language}. This variability underscores the need to conduct separate analyses of summary from various perspectives. In this paper, we adopt two intuitive perspectives—\textit{analytical} and \textit{narrative}—in accordance with our evaluation objectives, and we carry out the complete pipeline for each perspective. The definitions and distinctions of these two perspectives can be found in Table~\ref{tab:query-comparison}.

% \paragraph{Validation of the Key-fact Tree}


% \subsubsection{Key-fact Tree Generation}
% In this study, we propose the Key-fact Tree, a structured framework designed to extract and organize critical facts from each text chunk in a hierarchical way. We adopt this method to systematically evaluate an LLM’s ability to capture information at different levels of detail, as well as to quantify completeness and conciseness. The key-fact tree consists of three levels: Root, Branch, and Leaf. The \textit{Root} level key-fact represents the overarching purpose, main argument, or central idea of the text chunk. The \textit{Branch} level key-fact captures key supporting ideas, arguments, or major narrative developments that elaborate on or support the root. Finally, the \textit{Leaf} level key-fact contains specific evidence, minor details, or examples that provide further clarification or elaboration for each branch. These three levels maintain a clear logical relationship that enhances the delivery of both explicit and underlying information. By structuring facts hierarchically, the Key-fact Tree ensures that the flow of information—from broad concepts to detailed evidence—is coherent and comprehensive. To generate the Key-fact trees, we employ GPT-4o; the input to the model consists of a 4K-token excerpt from the original text(See Section~\ref{sec:source_data_prep}), combined with a perspective-tailored prompt, which is provided in the Table~\ref{tab:narrative_tree_generation} and Table~\ref{tab:analytical_tree_generation}.
% % These three levels maintain a clear logical relationship that improves the delivery of both explicit and underlying information. By structuring facts hierarchically, the key-fact tree ensures that the flow of information, from broad concepts to detailed evidence, is coherent and comprehensive.
% % Since large language models have demonstrated strong and effective capabilities in processing short texts (4K tokens), often performing at a level comparable to human comprehension, we employ GPT-4o to generate the key-fact trees. The input to the model consists of a 4K-token excerpt from the original text, combined with a perspective-tailored prompt, which is shown in the Appendix.


% \paragraph{Validation of the Key-fact Tree}

% % % To ensure the accuracy and reliability of the extracted key facts, 
% % Since LLM generated texts still suffer from hallucination, subjective inference, and redundancy\cite{Huang_2025}, we designed a comprehensive and rigorous automatic validation process to ensure the accuracy and reliability of the extracted key facts. This process assesses each key fact on three critical dimensions: faithfulness, subjectivity, and significance. The faithfulness evaluation focuses on detecting the factual error occurs in the key fact. The subjectivity evaluation is about judging if the key fact is inferenced total out of subjectivity without the solid evidence support. The significance evaluation meant to ensure all the key fact is crucial information about the context. 
% % For this validation, we use GPT-4o as the evaluator, leveraging tailored prompts to configure it as distinct validation agents for each dimension. 
% % % he evaluator is provided with both the original text chunk and the corresponding key-fact tree, and subsequently produces a validation tree.In this tree, each node represents a binary label indicating whether the corresponding key fact passes or fails the validation criteria.
% % The evaluator, given both the original text chunk and the corresponding key-fact tree, produces a validation tree where each node represents a binary label indicating whether the key fact passes or fails the validation criteria. 
% % Then the validation process follows a strict rule: if any one of the three labels is marked as invalid, the corresponding key-fact is considered an invalidated key-fact and is removed from the entire key-fact tree to keep all the remaining key facts accurate, objective, and significant. The detailed validation prompts used to configure GPT-4o for this multi-agent evaluation are provided in the appendix~\ref{appendix:keyfact_tree_validation_prompt}.To verify the reliability of this automatic validation process, we conduct human annotation on a sample of 500 validation trees across all three criteria. Three experienced annotators independently examine these validation labels.In this process, each annotator assesses whether they agree or disagree with each validation label. With this result, this automatic protocol of the key-fact creation can be proven to be reliable and scalable. 

% Despite significant advancements, LLM-generated content can still exhibit hallucinations, subjective inferences, and redundancy \cite{Huang_2025}, stressing the importance of verifying the key-fact trees produced by GPT-4o. Therefore,we design a comprehensive and rigorous automatic validation process to filter out the unqualified key facts,ensuring the accuracy and reliability of the extracted key facts. 
% In this process, each key fact is evaluated along three critical dimensions: (1) Faithfulness, to detect factual errors; (2) Subjectivity, to determine whether the fact is inferred solely on subjective grounds without robust evidence; and (3) Significance, to ensure that the fact provides essential information relevant to the context.
% For this validation, we use GPT-4o as the evaluator, leveraging tailored prompts to configure it as distinct validation agents for each dimension. The evaluator, given both the original text chunk(See Section~\ref{sec:source_data_prep}) and the corresponding key-fact tree, produces a validation tree where each node represents a binary label indicating whether the key fact passes or fails the validation criteria. Then the validation process follows a strict rule: if a key fact fails any of the three criteria-faithfulness, subjectivity, or significance-it is considered an invalidated and removed from the entire key-fact tree, thus keeping all the remaining key facts accurate, objective, and significant. The detailed validation prompts used to configure GPT-4o for this multi-dimension evaluation are provided in Table~\ref{tab:keyfact_tree_validation_faith} and Table~\ref{tab:keyfact_tree_validation_sig} and Table~\ref{tab:keyfact_tree_validation_subj}. We validate the effectiveness of this validation step with experienced annotators in Section~\ref{sec:humanval}.

% \subsection{Query Generation}
% In our query-focused summarization (QFS) task, queries must remain highly relevant, logically coherent, and well-aligned with the corresponding excerpt from the original novel. For each 4K-token chunk (see Section~\ref{sec:source_data_prep}), we employ GPT-4o to generate a query based on both the chunk itself and its associated key-fact tree, which provides a structured representation of the content. The prompts used for query generation are presented in Table~\ref{tab:narrative_query_generation} and Table~\ref{tab:analytical_tree_generation}. To ensure the validity of these queries and to further examine the feasibility and scalability of LLMs for query generation, three experts independently evaluate each query (see Section~\ref{sec:humanval}). Queries deemed too vague or misaligned with the chunk's context—thereby potentially affecting subsequent summarization steps—are re-generated to maintain clarity and effectiveness.




% \subsection{Summary Generation}
% To investigate how long-form generation capabilities vary across different model scales and architectures, we evaluate six representative LLMs. These range from commercial models (GPT-4o, GPT-4o Mini, Claude-3.5-Sonnet, and Claude-3.5-Haiku) to open-source alternatives (Llama-3.1-405B-Instruct and Llama-3.1-8B-Instruct), allowing for a direct comparison of both model architectures and parameter scales. Further model details are provided in Appendix~\ref{appendix:model_details}.

% In total, we generate 4,800 summaries (16 novels × 25 chunks × 2 perspectives × 6 summarizers), which are subsequently used in our multi-perspective, multi-dimensional evaluation.

% \subsection{Fine-grained Evaluation}
% Since a summary’s quality depends on multiple aspects—not only factual accuracy but also its completeness and conciseness—a single-dimensional assessment provides an incomplete picture. In addition, book-length summarization poses unique challenges, including increased risk of hallucination, omission of key information, and redundancy. To address these issues, we employ a multi-dimensional, fine-grained evaluation framework inspired by FineSurE \cite{song2024finesure}. Crucially, our pipeline reduces the complexity of lengthy source texts by segmenting each novel into 4K-token chunks (Section~\ref{sec:source_data_prep}), thus producing summaries of manageable length that can be evaluated in a fine-grained, multi-dimensional way. This chunk-level approach—combined with the Key-fact Tree for structured references—ensures that FineSurE delivers high-quality labels aligned with human judgment.

% We divide our evaluation into two main tasks: Fact Checking and Key-fact Alignment. The Fact Checking step focuses on detecting factual errors in summary sentences to gauge faithfulness. Specifically, we split each summary into individual sentences and prompt GPT-4o to label each sentence as either faithful or not, drawing on a taxonomy of error types (Table~\ref{tab:error-categories}). The Key-fact Alignment step addresses the completeness and conciseness of the summaries by checking how many critical facts (from the Key-fact Tree) are included, and how many sentences in the summary actually contain at least one key fact. Both steps benefit from the chunk-level scope, which ensures that reference passages are neither too large to overload the evaluation model nor too small to lose contextual coherence. Formulas for computing these metrics are provided in Appendix~\ref{appendix:eval_details}. Furthermore, we present human judgments of the evaluation results in Section~\ref{sec:humanval}, ensuring an additional layer of reliability and interpretability.

% % Since our pipeline uses long-form text generation task, for long-text evaluation, a single-dimensional assessment is insufficient to determine whether a summary is of high quality. Additionally, summary-level evaluation fails to present the results with a precise and concrete percentage.Therefore, we adopt a multi-dimension, fine-grained evaluation framework, following the existing framework\cite{song2024finesure}. Moreover, with the knowledge of which chunk each summary is from, we can use the original chunk text and the corresponding key-fact tree as the reference to conduct the evaluation. The evaluation is divided into two main tasks: Fact checking and Key-fact alignment. 

% % \paragraph{Fact checking}
% % The fact checking step is designed to evaluate the faithfulness of the summaries. Previous work has demonstrated that large language models are a cost-effective and reliable evaluation tool, we use GPT-4o as our evaluator. First, to ensure sentence-level, fine-grained assessment, we split the summary into individual sentences and evaluate them separately. Second, using the error taxonomy described in Table ~\ref{tab:error-categories}, we prompt LLM to generate the binary label indicating whether a summary sentence is faithful or not,along with the error type and the reason for giving the label. By providing both the error type and reasons, the LLM can be instructed in greater detail to produce more accurate evaluations, which also benefits subsequent human annotation. The formula of the calculation is provided in appendix~\ref{appendix:formula}

% % \paragraph{Key-fact alignment}
% % The key-fact alignment step is tailor to evaluate the completeness and conciseness of the summaries. Completeness is measured by counting how many key-facts are include by the summary. Conciseness is measured by counting how many summary sentences contain at least one key-fact. Using the key-fact tree as a reference, we can systematically identify which key facts should be present in an ideal summary. The evaluation follows these steps. First, we split summaries into sentences and assign an index number to each. Second, we prompt GPT-4o with the key-fact tree and the summary sentences to generate the binary label indicating whether each key-fact is contained, along with the index of the summary sentence index containing it. Finally, we compute the completeness and conciseness scores. The formula of the calculation is provided in appendix~\ref{appendix:formula}.
